Investigating the Relationship between Simulation Parameters and Flow Variables in Simulating Atmospheric Gravity Waves in Wind Energy Applications

Wind farms, particularly offshore clusters, are becoming larger than ever before. Besides influencing wind farms and local meteorology downstream, large wind farms can trigger atmospheric gravity waves in the inversion layer and the free atmosphere aloft. Wind farm-induced gravity waves can cause adverse pressure gradients upstream of the wind farm, that contribute to the global blockage effect, and favorable pressure gradients above and downstream of the wind farm that enhance wake recovery. Numerical modeling is a powerful means of studying wind farm-induced atmospheric gravity waves, but it comes with the challenge of handling spurious reflections of these waves from domain boundaries. Approaches like radiation boundary conditions and forcing zones are used to avoid the reflections. However, the simulation setup heavily relies on ad-hoc processes. For instance, the widely used Rayleigh damping method requires ad-hoc tuning to acquire a setup only applicable to a particular case. To surmount this hurdle, we conduct a systematic LES study for flow over a 2D hill and through wind farm canopies that explores the dependence of domain size and damping layer setup on parameters driving linearly stratified atmospheric flows. Mainly the internal waves in the free atmosphere reflect from the boundaries, therefore by simulation linearly stratified conditions we focus on internal waves only. The Froude number drives most of the internal wave properties, such as wavelengths, amplitude, and direction. Therefore, the domain sizing and Rayleigh damping layer setup mainly depends on the Froude number. We anticipated the effective wavelengths to be the correct length scale to size the domain and damping layer thickness. Also, the damping coefficient is scaled with Brunt-V\"ais\"al\"a frequency.

==> introduction_revised.tex <==
\introduction
\label{sec:intro}
 
 The size of a modern wind farm, especially offshore, can extend to several tens of kilometers, involving flow interactions on a regional scale and to great elevations into the free atmosphere. The energy and momentum extraction caused by a large wind farm is significant enough to decelerate the flow in the atmospheric boundary layer (ABL) \citep{Frandsen1992}, \citep{Smith2010}, which slowly recovers because of turbulent momentum transfer and the interplay of the large-scale driving pressure gradient and Coriolis effects. This is evident from the compound wake of large wind farms, which compared to small wind farm wakes, extend far beyond the wind farm in the streamwise direction. Generally, researchers study wind farm interactions with the ABL alone and not with the free atmosphere above, but a full understanding of large wind farm behavior requires an understanding of the farm's effect on the free atmosphere and vice versa.

The stability and temperature structure of both the ABL and the free atmosphere is deeply involved in the flow dynamics of large wind farms. For instance, the thickness of the ABL can significantly decrease during stable atmospheric conditions. In offshore environments in particular, the capping inversion, the relatively thin strongly stable layer that often forms between the ABL and the free atmosphere, can drop to a few hundred meters at night. In such conditions, wind farms can induce atmospheric gravity waves (AGWs), which include trapped gravity waves (TGWs) in the capping inversion and internal gravity waves (IGWs) in the free atmosphere aloft. Wind farm-induced AGWs were identified by \citet{Smith2010}, who analogized wind farms as semi-permeable obstacles that can deflect the flow upwards to displace the capping inversion, resulting in these buoyancy-driven waves. 

Wind farm-induced AGWs can affect wind farm performance by creating streamwise pressure gradients that accelerate or decelerate the flow into and through the farm, contributing to the phenomenon of "large wind-farm blockage" and affecting the way the compound wind-farm wake recovers. \cite{Smith2010}, \cite{Allaerts2018}, and \cite{Lanzilao2021} believe that AGWs cause the large wind-farm blockage effect at the entrance of a wind farm.  \citet{Wu2017} theorize that the large wind-farm blockage effect is the combined effect of AGWs and the cumulative turbine induction. The term ‘regional efficiency’ of wind farms was introduced by \citet{Allaerts2018a} to characterize the impact of atmospheric gravity waves on wind-farm performance. They claim that regional efficiency is of the same order wake-induced wind-farm efficiency losses. \citet{Allaerts2018} estimated a  $4$ to $6\%$ decrease in the annual energy production of an offshore wind farm caused by the global blockage created by AGWs. On the other hand, \citep{Lanzilao2022} and \citep{StipaEtAl2023a} argue that AGWs can also assist wind farm wake recovery because they can create a local favorable pressure gradient at the far end of and behind the wind farm. However, the extent of the favorable pressure and its positive effects on farm wake recovery are still unknown. Because of the sheer scale of AGWs and their interaction with wind farms, little if any experimental data exists to quantify their effects on wind farms; most investigations about wind-farm-induced AGWs are numerical.

Numerical flow simulation, particularly large-eddy simulation (LES), is currently a powerful approach to study AGWs. Gravity waves induced by large wind farms were first investigated with LES by \citet{Allaerts2017}. Since then, the major work on wind farm-induced gravity waves using LES was performed by \citet{2016_Allaerts_phdthesis}, \citet{Allaerts2015, Allaerts2017, Allaerts2018a}, \citet{Allaerts2018}, and \citet{Lanzilao2021, Lanzilao2022} using pseudospectral codes.  \citet{StipaEtAl2023a} and \citet{wes-2022-63} have also studied wind-farm-induced gravity wave effects using finite-volume codes.  

The simulation of wind-farm-induced atmospheric gravity waves on a finite domain requires special treatment at all domain boundaries other than the ground to stop the gravity waves from spuriously reflecting off of these boundaries that do not exist in reality.  AGWs propagate in all directions, so they will spuriously interact with the inflow, outflow, and top boundaries (all of which do not exist in reality).  Two main classes of methods exist to mitigate spurious AGW-domain boundary interaction: 1) "radiative" boundary conditions and 2) damping layers.

Radiative boundary conditions often take the form
\begin{equaton}
    \frac{\partial \phi}{\partial t} + c_j \frac{\partial \phi}{\partial n_j} = 0
\end{equation}
where $phi$ is the quantity being transported through a boundary with normal, $n_j$, and $c_j$ is wave transport velocity.  One way to imagine this boundary condition is that it attempts to set the transported quantity $phi$ exactly to the value the wave causes it to be as the wave propagates to the boundary.  The difficulty is determining $c_j$ or a good approximate of it.  This is often only possible in idealized situations.  The radiative boundary condition is capable of allowing wave energy out of the domain only if the waves are moving perfectly normal to the boundary \citet{Durran1999}. However, the waves are typically moving at an angle relative to horizontal.  

A popular alternative to the radiative boundary condition is the damping layer.  Damping layers, sometimes referred to as "sponge zones," attempt to attenuate waves as the wave moves through the zone.  These zones are placed adjacent to domain boundaries and have a prescribed thickness.  A downside to such zones is that because they have thickness, one has to increase the domain size to account for their thickness, which adds some extra cost.  Typically damping layers are either of the viscous type or of the relaxation type, also known as Rayleigh damping layers (RDLs).  RDLs appear much more commonly used than viscous damping, and in our experience, RDLs are more effective than viscous damping.  Also, a recent study by \citet{Lanzilao2022} found that RDLs outperform radiative boundary conditions in minimizing AGW reflections in wind farm simulations.  Therefore, we will focus on the RDL in this study.

In principle, the quantity of interest, usually velocity but also sometimes temperature, entering an RDL is relaxed towards a prescribed reference value at a specified time scale as the wave travels through the RDL, reflects off the boundary, and travels through the RDL once again. Rayleigh damping enters the transport equations as a forcing term which takes the form
\begin{equation}
    f^{RDL} = -\frac{1}{\tau}c[\phi - phi_{ref}]
\end{equation}
where $\phi$ is the field to be damped within the RDL.  For example, commonly the velocity field is damped, so $\phi$ = $U_i$ is driven towards $U_{{i}_{ref}}$, which could be defined as components of geostrophic wind.  Sometimes the situation is ageostrophic, and a reference horizontal velocity is not convenient, so only the vertical component of velocity is damped. The Rayleigh function, $c$, is the a critical part of RBL that ensures that the wave gradually dissipates energy as it travels through the RDL thickness. $c$ can be a linear, exponential, polynomial, or cosine function.  We use the cosine form given here for the upper boundary,
\begin{equation}
    c = [1- \cos(\frac{\pi}{s_\mathrm{ra}}{\frac{z - (L_\mathrm{z} - L_\mathrm{d})},{L_\mathrm{d}}})]
\end{equation}
where $z$ is the total height of the domain, $L_\mathrm{z}$ is the height of the non-damped region, $L_\mathrm{d}$ is the thickness of the damping layer, and $s_\mathrm{ra}$ is the damping fraction. The time scale, $\tau$, or damping coefficient controls how fast the quantity is relaxed toward a reference value. In a recent study by \citet{Lanzilao2022}, $1/\tau$ is scaled with the Brunt-V\"ais\"al\"a frequency (N) in pursuit of the optimal value for wind farm simulations, suggesting the value of $\xi = 1/\tau N$ to be 3. Whereas \citet{2016_Allaerts_phdthesis} tuned their RDL for optimal damping coefficient and used $1/\tau = 0.0001~s^-1$, translating into $\xi = 0.017$; they used the same value in most of their later studies including, \citet{Allaerts2017, Allaerts2018, Allaerts2018a}. The damping layer thickness is another essential RDL parameter as it determines the space available for the forcing to dissipate the incoming wave energy. \citet{klemp-Lilly1978} suggested the thickness to be more than one vertical wavelength of the wave. More recent studies also follow this convention but without any further investigation; \citet{2016_Allaerts_phdthesis}, \citet{Allaerts2017}, \citet{Allaerts2018}, and \citet{Lanzilao2021, Lanzilao2022} use a \SI{15}{\kilo\m} RDL only at the top boundary; the vertical wavelengths in their simulations were always less than \SI{15}{\kilo\m}. 

The damping fraction $s_\mathrm{ra}$ was considered one of the two most critical parameters by \citet{Lanzilao2022}, which determines the fraction of the damping layer where a cosine function is applied. If $s_\mathrm{ra}$ is $0.8$, the cosine ramp up/down of damping is used for $80\%$ of the layer, and damping strength in the remaining $20\%$ of the RDL is maximum. The damping function type is another aspect, which \citet{Peric} found less significant while investigating the approaches to dampen internal waves. We also think the damping fraction and type of damping function have little impact on effective damping.  Instead, the damping coefficient and thickness (collectively referred to as damping characteristics in this study) could be the most important RDL parameters. More importantly, no consensus and recommendations on properly tuning RDL are found in the literature. 

As mentioned above, many of the existing LES studies of wind farm interaction with AGWs are performed with codes that are horizontally pseudospectral.  Psuedospectral codes have the advantage of nearly exponential error convergence with increasing spatial resolution, but they come with the limitation that all lateral domain boundaries must be periodic.  This poses a challenge for wind farm simulations because we desire to feed turbulent ABL flow into the domain and allow that flow with the wind turbine wakes to exit the domain.  Periodic boundaries normally would cause the wake flow exiting the domain to reenter on the inflow side.  The solution to this problem is the introduction of a forcing fringe region adjacent to the downstream boundary which forces the waked solution back toward the precomputed or concurrently computed pure turbulent ABL inflow solution \citep{InoueEtAl2014}.  Finite-volume, finite-difference, and finite-element methods do not have this requirement of lateral periodicity and hence do not need a forcing fringe.  Inflow data is simply fed into the domain on the inflow boundary with a Dirichlet condition and the outflow boundary is often some sort of Neumann or advection boundary condition that lets the waked flow out.  There is no need for a fringe zone that forces the wake solution back to the inflow solution.  

We mention all of this because it is important to note that pseudospectral codes with their periodic lateral boundary conditions effectively have no lateral boundaries.  RDLs only have to be applied adjacent to the top boundary.  Furthermore, the forcing fringe used to force the downstream flow back toward the desired inflow state is a form of Rayleigh damping.  This means that AGWs will not reflect off of the lateral boundaries in pseudospectral LES, they will simply exit the domain on one side and reenter on the opposite side.  However, the forcing fringe will have some effect on damping their lateral progression or may trigger spurious gravity waves, requiring an additional treatment\citep{Lanzilao2021}.  

The more common finite-volume/difference/element codes have real lateral boundary conditions that gravity waves will either reflect off of or spuriously interact with.  Therefore, RDLs must be placed adjacent to these boundaries as well as adjacent to the top boundary.  Very little guidance is given in the literature for gravity wave treatment for lateral boundaries in finite-volume/difference/element codes. \citet{StipaEtAl2023a} and \citet{wes-2022-63} used FVCs for their large wind farm LES which are not restricted to horizontally periodic boundary conditions. The latter used true inflow and outflow boundary conditions, which is complicated when modelling AGWs. Any inconsistency between the inflow and the internal fields, triggers non-physical waves at the inlet which propagate into the domain over time. Besides spurious waves, reflection of gravity waves from the domain boundaries is a huge challenge. As shown in \Cref{fig:ref_vc}, the gravity waves triggered by a small hill under linearly stratified conditions should move up and out of the numerical domain. But the reality of a finite domain with boundary conditions that do not exactly depict the actual physical conditions at the boundaries cause these waves to reflect. The non-dissipated wave energy accumulates at the boundaries and propagates back into the domain because it never leaves the domain, eventually making the solution non-physical. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/example_refl.png}
    \caption{Vertical velocity contour of flow over a small hill located at x = 0 km. The region outside the red dotted box is Rayleigh damping layers at the inlet (left), top, and outlet (right).}
    \label{fig:ref_vc}
\end{figure}

These current approaches to setting up RDL in wind farm simulations are all ad-hoc. Extensive fine-tuning of the damping parameters is required to set up a working simulation applicable only to a specific case \citep{Lanzilao2022}. Thus, setting up reflection-free simulations becomes tedious, computationally expensive, and time-consuming. One way to make the process less ad-hoc is to investigate possible relations of simulation setup with physical parameters driving flows through wind farms under stable atmospheric conditions.

This study aims to propose a baseline to set up simulations involving internal atmospheric gravity waves. The focus is identifying flow parameters dictating internal wave properties such as wavelength and direction. We anticipate that appropriate domain length, height, and damping layer thickness are related to the effective wavelengths, and the damping coefficient relates to the buoyancy frequency. By investigating the link between the internal wave properties and the simulation setup, we aim to propose recommendations for wind farm simulation set up under stable atmospheric conditions. As a starting point and for simplicity, we consider only the free atmosphere with a range of Froude Number (Fr) practical to wind farm applications. Investigating the free atmosphere separately is vital to handle the reflections, as the AGWs reflect off the boundaries. To this end, we consider two flow scenarios: first, we simulate flow over a bell-shaped 2D hill; second through wind farm canopies as surrogates of wind farms. We also use the analytical flow solution over the hill, mainly to validate the simulations and to understand the dependence of AGW properties on the identified flow parameters, i.e. Froude number.    

The remaining part of this paper is structured as follows: \Cref{sec:flow_sce} gives the flow scenarios studied in this research. In \Cref{sec:methodology}, the methodology used to carry out this study and the methods used to analyze the LES data are described. The numerical models and setups for the hill and wind farm canopy cases are also explained in this section. \Cref{sec:results_woa} presents the results, discussed under various sub-sections based on addressing the dependence of reflections on parameters identified critical to model IGWs. Likewise, \Cref{sec:results_wc} gives the results tested with the wind farm canopy.  In \Cref{sec:conclu}, the conclusions of this research are presented as initial recommendations to set up simulations involving atmospheric gravity waves. 
